ScalAna: Automating Scaling Loss Detection with Graph Analysis

Scaling a parallel program to modern supercomputers is challenging due to inter-process communication, Amdahl's law, and resource contention. Performance analysis tools for finding such scaling bottlenecks either base on profiling or tracing. Profiling incurs low overheads but does not capture detailed dependencies needed for root-cause analysis. Tracing collects all information at prohibitive overheads. In this work, we design ScalAna that uses static analysis techniques to achieve the best of both worlds - it enables the analyzability of traces at a cost similar to profiling. ScalAna first leverages static compiler techniques to build a Program Structure Graph, which records the main computation and communication patterns as well as the program's control structures. At runtime, we adopt lightweight techniques to collect performance data according to the graph structure and generate a Program Performance Graph. With this graph, we propose a novel approach, called backtracking root cause detection, which can automatically and efficiently detect the root cause of scaling loss. We evaluate ScalAna with real applications. Results show that our approach can effectively locate the root cause of scaling loss for real applications and incurs 1.73% overhead on average for up to 2,048 processes. We achieve up to 11.11% performance improvement by fixing the root causes detected by ScalAna on 2,048 processes.

==> ZeusMP_Teng.tex <==
\subsection{Case Studies on Real Applications}

In this section, we describe the experimental evaluation on real applications by using \ourtool to diagnose scaling issues and then optimize the code that causes scalability problems. The representative case studies include Zeus-MP, Nekbone, CloverLeaf, SST, and Sweep3d.

\subsubsection{Zeus-MP}
Zeus-MP is evaluated with a certain size of 64*64*64 by increasing the number of parallel MPI processes from 4 to 128. We observed that the scaling loss appeared when the number of parallel processes reaches 64. \ourtool is then applied to diagnose the problem, compared with two state-of-the-art tools, Scalasca~\cite{geimer2010scalasca} and HPCToolkit~\cite{adhianto2010hpctoolkit}. 

%We first use \ourtool to generate a \ppg for Zeus-MP with 1.37\% runtime overhead and 181KB space cost. As shown in figure~\ref{fig:zeusmp-overhead}, Scalasca~\cite{geimer2010scalasca} generates more than 1TB traces with more than 10000\% runtime overhead (with I/O) at a function level, and HPCToolkit~\cite{adhianto2010hpctoolkit} produces 20MB profiling data with 1.32\% runtime overhead. Besides, \ourtool shows better scalability both in runtime and space overhead.

\textbf{Scaling Loss Detection and Optimization:} \ourtool first generate a \ppg and then performs backtracking algorithm on the graph to identify the root causes automatically. 
Figure~\ref{fig:zeusmp-backtracking} shows how \ourtool diagnoses the scaling issues on the \ppg of Zeus-MP by its backtracking algorithm. The vertical axis from top to down represents the dataflow, and the horizontal axis represents the parallel processes. The small points represent the vertices with normal performance while the circle points represent problematic vertices with abnormal performance on the same code snippets.
The arrows show how the backtracking paths based on intra- and inter-process dependences. 


In detail, the \texttt{MPI\_Allreduce} vertices at \textit{nudt.F:1473} are detected as scaling issue vertices due to the poor scalability of its execution time. %as shown in the bottom of figure~\ref{fig:zeusmp-backtracking}.
As shown in the bottom of figure~\ref{fig:zeusmp-backtracking}, the red lines track backward from the abnormal \texttt{MPI\_Allreduce} vertices, then go through the intra-process dependences of control/data flow and inter-process dependences of point-to-point(P2P) communications at \textit{nudt.F:1146,943,656}. 
Finally, the \texttt{LOOP} vertices at \textit{nudt.F:412} (top row in figure~\ref{fig:zeusmp-backtracking}) are identified as the root causes of scaling issues. 
We find the underlying reason is that only some of the processes need to execute the \texttt{LOOP} at \textit{nudt.F:412} while the others perform the non-blocking point-to-point communication at \textit{nudt.F:656}. 
Delays in these processes propagate through the non-blocking P2P communications at \textit{nudt.F:943} and \textit{nudt.F:1146}. 
The \texttt{MPI\_Allreduce} at \textit{nudt.F:1473} needs to synchronize all processes, so these delays cause the poor scalability of Zeus-MP. 
To fix the root causes identified by \ourtool, further parallelism for the \texttt{LOOP} at \textit{nudt.F:412} is applied to utilize the CPU resource from other waiting processes.  
Similarly, \ourtool detect another root cause of the scaling loss from the \texttt{LOOP}s at $\textit{hsmoc.F:123,423,534}$. 
The load/store instruction count and the cache miss count recorded by PMU keeps high with the increasing number of process. 
We use loop tiling and scalar promotion to reduce the cache miss and memory access. 
With those optimization, Zeus-MP speeds up by 9.55\% on 128 processes, and the parallel efficiency is improved by 9.61\%.

As for other state-of-the-art tools, Scalasca could detect the function-level root causes by tracing. 
While the profiling-based HPCToolkit could only automatically detect the fine-grained loop-level scaling issues,
it still needs a lot of human efforts to detect the root causes of scaling loss.

\textbf{Performance and Storage Analysis:}
Figure~\ref{fig:zeusmp-overhead} shows the performance and storage analysis of \ourtool against the state-of-the-art Scalasca and HPCToolKit. The lower is better for both figure~\ref{fig:zeusmp-overhead}(a) and \ref{fig:zeusmp-overhead}(b). As for performance, both \ourtool and HPCToolKit keeps an ignorable level of runtime overheads by 1.37\% and 1.32\%, respectively.  
However, the tracing-based Scalasca needs more than 10000\% runtime overhead (with I/O) to generate the trace. 
As for storage, our light-weight \ourtool keeps better than both Scalasca and HPCToolKit. \ourtool only need 181KB space cost, while Scalasca generates more than 1TB traces and HPCToolkit produces 20MB profiling data.
The space costs of \ourtool is small and scalable due to it has nothing to do with runtime and is mainly related to program structure.

%\textbf{Summary:}


==> ack.tex <==
\section*{Acknowledgments}
We would like to thank the anonymous reviewers for their insightful comments. We thank Zhen Zheng, Liyan Zheng, Huanqi Cao, Bowen Yu, Guanyu Feng, Kezhao Huang, Shengqi Chen, and Jiaao He for their valuable feedback and suggestions. 
This work is supported by the National Key R\&D Program of China (Grant No. 2016YFB0200100), National Natural Science Foundation of China (Grant No. 61722208), Beijing Natural Science Foundation (4202031).
This work is supported in part by the China Postdoctoral Science Foundation (Grant No. 2020TQ0169), and the ShuiMu Tsinghua Scholar fellowship (2019SM131). 
Jidong Zhai is the corresponding author of this paper (Email:zhaijidong@tsinghua.edu.cn)
%Jidong Zhai is the corresponding author of this paper (Email: \href{mailto:zhaijidong@tsinghua.edu.cn}{\nolinkurl{zhaijidong@tsinghua.edu.cn}}).
\balance

==> copy.tex <==

\section{NPB-CG with Manually Injected Bottleneck}
%\label{sec:moti}
\label{sec:overview}

\begin{figure}[ht]
    %\vspace{-0.5em}
	\centering
	\includegraphics[width=\linewidth]{figures/cg-comm-pat.pdf}
	\caption{Program structure of NPB-CG and communication pattern in 8 processes}
	\label{fig:cg-comm-pattern}
	\vspace{-0.5em}
\end{figure}

\begin{figure}[ht]
    %\vspace{-0.5em}
	\centering
	\includegraphics[width=\linewidth]{figures/cg-inject-hpctrace.pdf}
	\caption{HPCToolkit's \textit{hpctraceviewer} for a NPB-CG run in class C with 8 processes}
	\label{fig:cg-inject-hpctrace}
	%\vspace{-0.5em}
\end{figure}

\begin{figure*}[ht]
    %\vspace{-0.5em}
	\centering
	\includegraphics[width=0.7\textwidth]{figures/cg-inject-hpcviewer.pdf}
	\caption{HPCToolkit's \textit{hpcviewer} for a NPB-CG run in class C with 8 processes}
	\label{fig:cg-inject-hpcviewer}
	\vspace{-0.5em}
\end{figure*}

\begin{figure}[t]
    %\vspace{-0.5em}
	\centering
	\includegraphics[width=0.8\linewidth]{./figures/cg-motivation-scalana.pdf}
	\caption{process 4 communication dependence}
	\label{fig:cg-insert-scalana}
	%\vspace{-1em}
\end{figure}

We start by illustrating \ourtool's motivation and contribution with NPB-CG~\cite{npb} as an illustrating example.

We manually inject a fix workload code snippet in one process as a scalability bottleneck after an \texttt{MPI\_Send}. 
We run \nre in class D with different process numbers on TH2-system. 
And the result shows that the manually injected bottleneck causes a scaling loss (1024 processes is 49.42 seconds vs. 2048 processes is 49.53 seconds). 
Further analysis is needed to identify the scalability bottlenecks.

Tracing-based approaches like Scalasca~\cite{geimer2010scalasca} and Vampir~\cite{nagel1996vampir} use instrumentation technique to acquire event traces. 
Event traces contain the intra- and inter-process dependence that allow to pinpoint the root causes.
However, it is estimated by small-scale experiments that the time overhead of Scalasca is over 250GB in 1024 processes. 
Time and space costs are prohibitive at large scale, which hinders its analysis of large-scale parallel programs. 

Sampling-based tools like HPCToolkit~\cite{adhianto2010hpctoolkit} achieve very low overheads. 
It provides both tracing and profiling GUIs: hpctraceviewer and hpcviewer. 
Due to the space limit, we use \nre in 8 processes to show them.
Figure~\ref{fig:cg-inject-hpctrace} shows a screenshot of HPCToolkit's hpctraceviewer. 
The time of MPI\_Wait in most processes and the time of MPI\_send in process 2 is longer than process 4. 
However, it is difficult to identify the root causes of the increasing of the MPI time.  
Figure~\ref{fig:cg-inject-hpcviewer} shows the result of HPCToolkit's hpcviewer. 
In the figure, the left part is \textit{hpcviewer} result of CG.D.1024 while the right part is CG.D.2048. 
We use Coarfa's work~\cite{coarfa2007scalability} to diagnose scaling issues. 
In their work, if a node \textit{n} has comparable positive values for the excess work for inclusive and exclusive costs then the loss of scaling dues to \textit{n}.
And the nodes in the red circle have comparable values and both excess works for inclusive and exclusive costs (the time percentage in CG.D.2048 minus the time percentage in CG.D.1024) is positive. 
Therefore, these nodes are considered to be the scalability bottlenecks.
But node in the blue circle, which corresponds to the manually injected code snippet, is not considered to be a scalability bottleneck. 
Because sampling miss some inter- and intra-process dependence, the root cause of the scalability problem cannot be tracked easily in this case. 

Therefore, we present \ourtool to identify the root causes with inter- and intra-process dependence and keep low overhead. 
Figure~\ref{fig:cg-insert-scalana} shows the communication dependence and data dependence of CG in 8 processes. 
The colored edges are the propagation paths caused by communication dependence from manually injected computation in process 4. 
In our approach, we use the defective vertex detection and a backward propagation algorithm to track backward between the processes, then we can identify the scalability bottleneck in process 4 as the root cause. 
